Focal Split: Untethered Snapshot Depth from Differential Defocus

We introduce Focal Split, a handheld, snapshot depth camera with fully onboard power and computing based on depth-from-differential-defocus (DfDD). Focal Split is passive, avoiding power consumption of light sources. Its achromatic optical system simultaneously forms two differentially defocused images of the scene, which can be independently captured using two photosensors in a snapshot. The data processing is based on the DfDD theory, which efficiently computes a depth and a confidence value for each pixel with only 500 floating point operations (FLOPs) per pixel from the camera measurements. We demonstrate a Focal Split prototype, which comprises a handheld custom camera system connected to a Raspberry Pi 5 for real-time data processing. The system consumes 4.9 W and is powered on a 5 V, 10,000 mAh battery. The prototype can measure objects with distances from 0.4 m to 1.2 m, outputting 480$\times$360 sparse depth maps at 2.1 frames per second (FPS) using unoptimized Python scripts. Focal Split is DIY friendly. A comprehensive guide to building your own Focal Split depth camera, code, and additional data can be found at https://focal-split.qiguo.org.

==> sec/1_intro.tex <==
\section{Introduction}
% Start out by saying exactly what we did
% i.e. "we made this cool thing"
% look at gameboy paper

% Make sure to mention that computation is at the edge, unlike some previous work.

% Another subsection in related work 

% Then establish utility of depth images broadly in computing and CV.



Since their introduction to computer vision, depth images have proven to be broadly useful across disciplines. There are a number of methodologies for collecting depth images with each having its own tradeoffs with respect to range, accuracy, robustness, and SWaP-C (size, weight, power, and cost), as shown in Figure~\ref{fig:TODO}.

% \johncomment{Establish the existence of a menagerie of depth imaging techniques. Emphasize that each has its strengths and weaknesses; that each is appropriate for a different application. }
% \johncomment{Our storytelling direction is that we have refined and adapted an existing technique to fill an as-yet-unfilled niche in depth imaging.}
% I imagine that a really good figure for this would be a technology trade off plot (this is a good example: (https://ojoyoshidareport.com/wp-content/uploads/2024/04/Figure-1-1.png))

Many applications already have appropriate techniques for collecting depth images: with its high performance, large range, and high SWaP-C, LiDAR imaging is suitable for autonomous vehicles; structured light cameras are appropriate for more cost-sensitive applications with lower performance requirements; and stereo vision is appropriate for applications that require more robust depth sensing in environments with high ambient light, and it has a higher computational cost, requiring more sophisticated algorithms for disparity mapping and depth estimation. However, no method that we know of is appropriate for mobile depth imaging for extremely energy-sensitive applications.

% \johncomment{TODO: discuss background of DFDD; briefly explain shortcomings.}
Recently, a series of studies have focused on developing low-power, passive lighting depth sensors using the depth from defocus (DfD) technique. DfD extracts 3D information from images by modeling defocus blur. Recent DfD depth sensors demonstrate that they can use two input images to achieve a floating point operations per output pixel (FLOPOP) as low as 600 \cite{guo2017focal}, compared to approximately 7,000 FLOPOP required by efficient stereo depth-sensing algorithms \cite{rotheneder2018performance}. Using defocus in a monocular system has recently been shown to be a viable technique for generating depth images by a simple pixel-wise calculation with two image derivatives:

\begin{align}
    Z =& \frac{a}{b+I_{\rho}/\nabla^2 I}
    \label{eq:general_form},
\end{align}

Although DfD methods offer the advantage of lower computational cost, several challenges remain. One key challenge is the reliance on sequential shots to capture images and calculate depth maps. This means that a moving object can introduce noise into the calculations, depending on the distance the object moves between frames.

In this paper, we introduce a novel depth sensor called the Snapshot Hand-Held Depth from Defocus Camera, designed to overcome issues associated with sequential shots by capturing two images simultaneously. We enhance the image formation model and present a new theory that enables depth map calculation using two images captured by cameras with different flange focal distances. Unlike previous Depth from Differential Defocus (DfDD) methods, our approach captures images concurrently, eliminating concerns about motion-induced noise and the need for additional devices, such as an electric tunable lens (ETL), to adjust optical power. In contrast to stereo vision systems, which require multiple cameras and entail high computational costs for image matching, our method achieves depth sensing with minimal power requirements. We demonstrate that our approach is both low-power and robust against motion-induced errors.

% \johncomment{TODO: Discuss improvements of this work, i.e. robustness to motion, improvement in SWap-C}
% \johncomment{TODO: Explain how systems inspired by this work will have a major impact across application spaces}

% \subsection{Contributions}

% \johncomment{TODO: describe contribution list for this work}
% Depth from defocus: any algorithm that uses 
% DFDD specifically is a computationally inexpensive class of algorithms. 
% Just like with optical flow, there are cheap and expensive methods for depth from defocus. Depth from Defocus can use 
% Optiall

The contribution of this paper can be summarized as follows:

\begin{enumerate}
    \item  \textbf{Theory for new optomechanical setup.} We present a novel image formation model and a depth from differential defocus theory that enable depth map calculation from input images with different pinhole projections.
    \item \textbf{Reduction in power consumption.} We adapt the new DfDD theory to a low-power single-board computer platform, showing that DfDD can be computed in a power budget $\leq$ 10W.
    \item \textbf{Optomechanical setup for snapshot imaging. } We introduce a beamsplitter to a novel optical setup that allows for the simultaneous capture of images with differential focus.
\end{enumerate}

\label{sec:intro}

% Discussion of applications can go in the intro.
%
% Adding a new feature space to a tye of imaging system.
% Look at existing applications that could benefit.
% Look at new applications that didn't exist before.
%  - AR: activity and object recognition
%  - Security / Surveillance
%  - Conservation?

==> sec/tbl_performance_compare.tex <==
    \centering
    \begin{tabular}{llllccc}
        \toprule
        \textbf{Work} &             \textbf{Technique}           & \textbf{Compute}                        & \textbf{Resolution} & \textbf{Untethered?} & \textbf{Real Time?} & \textbf{Snapshot?} \\
        \midrule
        Newcombe et. al, 2011~\cite{newcombe2011dtam}    & SfM        & i7 workstation with NVIDIA GTX 480 GPU  & 640 $\times$ 480           & \xmark               & \cmark              & \xmark             \\
        Sch{\"o}nberger et. al, 2016~\cite{schonberger2016structure}  & SfM        & Unspecified desktop workstation         & variable            & \xmark               & \xmark              & \xmark             \\
        Tang et. al, 2017~\cite{tang2017depth}         & DfD           & Dual 8-core Xeon Server                 & 5184 $\times$ 3456 and 2464 $\times$ 3280 & \xmark       & \xmark              & \xmark             \\
        Alexander et. al, 2018~\cite{alexander2018focal}    & DfDD & i7 6820HK notebook with NVIDIA GTX 1080 GPU & 300 $\times$ 480    & \xmark               & \cmark              & \xmark             \\
        This Work                      & DfDD & Raspberry Pi 5                       & 640 $\times$ 480                & \cmark               & \cmark              & \cmark             \\
        \bottomrule
    \end{tabular}


    % \centering
    % \begin{tabular}{llllccc}
    %     \toprule
    %     \textbf{Work} &             \textbf{Technique}           & \textbf{Compute}                        & \textbf{Resolution} & \textbf{Untethered?} & \textbf{Real Time?} & \textbf{Snapshot?} \\
    %     \midrule
    %     Newcombe et. al, 2011     & Structure from Motion        & i7 workstation with NVIDIA GTX 480 GPU  & 640 x 480           & \xmark               & \cmark              & \xmark             \\
    %     Schonberger et. al, 2016  & Structure from Motion        & Unspecified desktop workstation         & variable            & \xmark               & \xmark              & \xmark             \\
    %     Tang et. al, 2017         & Depth from Defocus           & Dual 8-core Xeon Server                 & 5184 x 3456 and 2464 x 3280 & \xmark       & \xmark              & \xmark             \\
    %     Alexander et. al, 2017    & Differential Depth from Defocus & i7 6820HK notebook with NVIDIA GTX 1080 GPU & 300 x 480    & \xmark               & \cmark              & \xmark             \\
    %     Ours                      & Differential Depth from Defocus & Raspberry Pi 5                       & xxxx                & \cmark               & \cmark              & \cmark             \\
    %     \bottomrule
    % \end{tabular}
